Synapse: Interactive Guidance by Demonstration with Trial-and-Error Support for Older Adults to Use Smartphone Apps

As smartphones are widely adopted, mobile applications (apps) are emerging to provide critical services such as food delivery and telemedicine. While bring convenience to everyday life, this trend may create barriers for older adults who tend to be less tech-savvy than young people. In-person or screen sharing support is helpful but limited by the help-givers' availability. Video tutorials can be useful but require users to switch contexts between watching the tutorial and performing the corresponding actions in the app, which is cumbersome to do on a mobile phone. Although interactive tutorials have been shown to be promising, none was designed for older adults. Furthermore, the trial-and-error approach has been shown to be beneficial for older adults, but they often lack support to use the approach. Inspired by both interactive tutorials and trial-and-error approach, we designed an app-independent mobile service, \textit{Synapse}, for help-givers to create a multimodal interactive tutorial on a smartphone and for help-receivers (e.g., older adults) to receive interactive guidance with trial-and-error support when they work on the same task. We conducted a user study with 18 older adults who were 60 and over. Our quantitative and qualitative results show that Synapse provided better support than the traditional video approach and enabled participants to feel more confident and motivated. Lastly, we present further design considerations to better support older adults with trial-and-error on smartphones.

==> Introduction-Old.tex <==

\section{Introduction}
Wireless technology and smart phones are developing rapidly over the last decades. Accordingly, the number of smartphone users is rising over years, across different age groups~\cite{SmartphonesUsers:online}.
However, compared to younger adults, older adults, who are gradually taking up a larger proportion of human beings~\cite{WHO} still show a lower acceptance of smartphones~\cite{US:online, UK:online, BerenguerAnabela2017ASUA}. In addition, owning a smart phone does not necessarily mean that having adopted the full capabilities of a smartphone. An in-depth survey study conducted by Berenguer et al. pointed out that the older adults who do adopt smartphones tend to use them as feature phones and do not adopt services that are popular among younger users~\cite{BerenguerAnabela2017ASUA}.

% apps benefit for older adultsPrevious studies have shown positive impact for older adults to use mobile applications, which have potential to improve their quality of life and maintain their independence for middle-aged and older people. Previous studies suggest positive impact of mobile applications for older adults―improving their quality of life and maintaining their sense of independence (Plaza et al., 2011) (Leung et al., 2012).

The possible explanations of the age-related differences in smartphone usage includes the ageing physical and cognitive ability(e.g., vision impairment, declined mental status)~\cite{Mohadis2014ASUB, Pang2015OAADS}, the lack of knowledge on how to use, or about the smartphone~\cite{Mohadis2014ASUB, Pang2015OAADS}, pointing out that older adults may need help in adopting and using smartphones. 

Indeed, according to Pew Research Center, a significant majority of older adults report that they need assistance when it comes to using new digital devices and 77\% indicate they would need to be helped walk through the process by someone else~\cite{Pew14:online}. Moreover, social support has been considered to be important in both the appropriation and the disappropriation of smartphones. Pang et al. revealed that participants who adopt smartphones still keep searching social help for certain functions during the use of smartphones, and participants who reported disappropriation were living alone and had infrequent interactions with their neighbors, implying little external help from other smartphone users~\cite{Pang2015OAADS}. While in person help may not always be available. According to the United Nations, more and more older adults live independently, making it even more difficult for them to get efficient help from their children or other relationship~\cite{UN17Arrangement}. 

Therefore, there is a crucial need for enabling older adults to get help remotely in order to get a broader social help. While remote assistance is challenging. Typical solutions for guiding a remote user to use smartphones such as phone calls, or written instructions via email seems to be useful, however, they may lead to communication issues between the help-giver and the help-seeker, due to the lack of shared visual screen and the misunderstanding of terminologies probably used during the instruction. Although some video tutorials are available, these are fast-paced and hard to follow for those who had little acquaintance with smartphones. Although approaches such as Pause and Play enables the video to automatically pause and play to stay in sync with the user~\cite{Pongnumkul2011}, and MixT combined the static and video clips together to provide a more effective tutorials~\cite{Chi2012Mix}, these tutorials are not situated within the tool itself, making it frustrating for users to switch back and forth between the task and the tutorial~\cite{Pongnumkul2011}. More extend, another approach of adding an interactive user guide when the user firstly launches the app alleviates the lack of visual context to some extent. However, only a few UI elements could be highlighted with a brief animation of gestures, which would be inefficient and difficult to comprehend for inexperienced users like older adults. Methods such as adding live screen or video sharing support, and using third party applications like InkWire~\cite{InkWire}, TeamViewer~\cite{TeamViewer}, or AirDroid~\cite{AirDroid} to remotely control the Android device appear to solve the visual shared problem, while these approaches require the help to be synchronous, which add restrictions to the remote help since the help-giver and the help-seeker may likely have different schedules. Moreover, these approaches would not work well without stable and high bandwidth network connection and also violate user’s privacy. Vyas et al. further developed the remote assistance with an app called APPAmigo by capturing and recording the events from one device and recreate them in the other device to avoid getting complete access to control the entire remote device~\cite{Vyas2019AppAmigo}. While informative, the approach focus on the problem solving in a shortcut instead of motivating older adults to learn smartphones in a long term perspective. %Moreover, this kind of approach may let users lean to depend on the help givers gradually, which contradicts the willingness of being independent among older adults. 
Contextual tools like Sketch-sketch Revolution ~\cite{Jennifer2011Sketch-Sketch} and DemoWiz ~\cite{Chi2014DemoWizRS} offers either in-application interactive tutorials or within-context features, while most of them are application-dependent.
Furthermore, EverTutor was developed as an app which could provide a contextual interactive step-by-step guidance on smartphones by demonstration universally~\cite{Wang2014EverTutor}.
A more recent design Remo proposed by Aftab et al. allows help-givers to generate interactive tutorials by demonstration to provide remote help asynchronously~\cite{Remo}. %However, Remo did not provide a continuous communication between the help-giver and the help-seeker such as enabling the help-seeker to report the issues or raise questions during the usage of the tutorials.Like AppAmigo, Remo also lacks the ability to generalize tutorials that produce similar tasks. Besides,
However, Remo is presented as a design model with the limitation in assisting users with web pages. More importantly, few studies seriously consider the need of older adults during the design and development of the remote assistance app on smartphone usage with the single visual guidance.

Additionally, trial\&error is a typical way to learn in many domains~\cite{kavanaugh2019just}, and has also been proven to have benefits for older adults in source memory and episodic memory~\cite{cyr2012trial, cyr2015mistakes}. However, older adults face challenges when doing trial\&error such as lack of encouragement for self-diagnosis~\cite{fan2018guidelines}, and showed less preference in using trial\&error~\cite{mitzner2008older, Leung2012}. While, a previous research suggested that older adults may be more willing to try if they are supported to be more confidence that errors would not lead to severe consequences~\cite{barnard2013learning}. 
Therefore, we raise two research questions:
\begin{itemize}%[leftmargin=*]
\item {RQ1}:  Would the multimodal interactive tutorial better help older adults learn smartphones than the video?
%How do older adults use physical and digital banking platforms and what are the pros and cons of these platforms?
\item {RQ2}: Would the one with trial and error support better help older adults learn smartphones than the video?
\end{itemize}
To answer the research questions, we developed “Synapse", an app which create multimodal interactive tutorials by demonstration with "Basic mode" and "Trial\&Error mode" for older adults. We further conducted a controlled laboratory experiment containing interview with 18 older adults who are 60 and over to compare the performance and user experience between the traditional video, Synapse (Basic), and Synapse (Trial\&Error). As AR technology evolves these days, and approaches such as Anicode~\cite{Wang2019Anicode} and Dynamics 365 Remote Assist~\cite{Dynamics365}, we following asked their attitude, opinions about the related technology. As a summary, we made following contributions:
\begin{itemize}%[leftmargin=*]
\item {1}:  We developed a novel interactive remote application "Synapse" with "Basic mode" and "Trial\&Error mode" to better support older adults to learn smartphones, which are proven to be beneficial to them.
%How do older adults use physical and digital banking platforms and what are the pros and cons of these platforms?
\item {2}: We identified typical types of errors older adults often make during the trial\&error approach.
\item {3}: 
\end{itemize}


==> LimitationsFutureWork.tex <==
\section{Limitations and Future Work}

app location, size 

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

